GAPX: Generalized Autoregressive Paraphrase-Identification X

Paraphrase Identification is a fundamental task in Natural Language Processing. While much progress has been made in the field, the performance of many state-of-the-art models often suffer from distribution shift during inference time. We verify that a major source of this performance drop comes from biases introduced by negative examples. To overcome these biases, we propose in this paper to train two separate models, one that only utilizes the positive pairs and the other the negative pairs. This enables us the option of deciding how much to utilize the negative model, for which we introduce a perplexity based out-of-distribution metric that we show can effectively and automatically determine how much weight it should be given during inference. We support our findings with strong empirical results.

==> intro_bak.tex <==

\section{Introduction}
Paraphrases are sentences or phrases that convey the same meaning using different wording \citep{10.1162/COLI_a_00166}, and is fundamental to the understanding of languages. Paraphrase Identification is the important task of identifying if a given pair of sentences has the same meaning, and has many important downstream applications such as summarization, machine translation \citep{DBLP:journals/corr/abs-1904-09675}, and question-answering \citep{cer-etal-2017-semeval}.

\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{negative examples.pdf}
    \caption{Negative samples in different datasets are mined differently in different datasets, and can lead to significant biases during training.}
    \label{linregintro}
\end{figure}

Recently, researchers have observed that neural network architectures trained on different datasets could achieve state-of-the-art performances for the task of paraphrase identification \citep{DBLP:journals/corr/WangHF17, DBLP:journals/corr/abs-1810-04805, DBLP:journals/corr/abs-2104-14690}. While these advances are encouraging for the research community, it has however been observed that these models can be especially fragile in the face of distribution shift \citep{shen-lam-2021-towards}. In other words, when a model trained on a source dataset $\mathcal{D}^s$ is tested on another dataset, $\mathcal{D}^t$, collected and annotated independently, and with a distribution shift, the classification accuracy drops significantly \citet{DBLP:journals/corr/abs-1904-01130}. %In fact, \citet{DBLP:journals/corr/abs-1904-01130} has observed that adversarial samples can even degrade the model's performance to around the chance level (50\%). \red{Yifei: I think we are safe to say just in some extreme cases in stead of adversarial samples to avoid confusions, since this dataset is not strictly adversarial per say.}

%Previous works have shown that the lack of generalization caused by distribution shift can be attributed to the issue of shortcut learning \citep{DBLP:journals/corr/abs-1803-02324, DBLP:journals/corr/abs-2004-07780}, where ``clues'' specific to the training dataset introduced in the process of dataset collection and annotation are picked up by the model. Because these shortcut features are specific to the training set, it becomes quite challenging for the model to generalize to real-world out-of-distribution scenarios. Researchers \citep{DBLP:journals/corr/abs-2103-06922, DBLP:journals/corr/abs-1908-10763, DBLP:journals/corr/abs-1909-03683} have proposed methods to identify training samples that can lead to the learning of shortcut features. By reducing the reliance of their models on these shortcut features that were detected, they were able to demonstrate improved generalization in many NLP problems like Natural Language Inference tasks and Vision Question Answering. Their methodology however depends on hand-picking shortcut features from known dataset bias \citep{DBLP:journals/corr/abs-1909-03683}, which is sometimes inadequate and even impractical. This is especially true for paraphrase identification, whereby finding the specific dataset bias feature learnt by black-box paraphrase identification models can prove to be quite challenging.

This paper presents our findings and observations that negative samples (i.e., non-paraphrase pairs) in the training set, as opposed to the positive samples, do not generalize well to out-of-distribution test samples. Intuitively, negative samples only represent a limited perspective of how the meanings of sentences can be different (and indeed it is practically infeasible to represent every possible perspective). We conjecture that negative samples are so specific to the dataset that they adversely encourage the model to learn biased representations. We show this observation in Figure~\ref{linregintro}. Quora Question Pair (QQP) \footnote{https://quoradata.quora.com/First-Quora-Dataset-Release-Question-Pairs} extracts its negative samples from similar topics. Paraphrase Adversarials from Word Scrambling (PAWS) \citet{DBLP:journals/corr/abs-1904-01130} generate negative samples primarily from word swapping. World Machine Translation Metrics Task 2017 (WMT) \citep{Bojar2017ResultsOT} considers negative examples as poor machine translations. We therefore hypothesize that biases introduced by the different ways negative samples are mined are major causes of the poor generalizability of paraphrase identification models.


Based on this observation, we would like to control the reliance on negative samples for out-of-distribution prediction. In order to achieve this, we propose to explicitly train two separate models for the positive and negative pairs (we will refer to them as the positive and negative models respectively), which will give us the option to choose when to use the negative model. \yifei{Since fitting to the distribution of positive samples and negative samples neglect the interplay between positive and negative samples, we train an additional discriminative model to capture the interplay. For in-distribution samples, we will use the positive, the negative models, and the discriminative model, while for out-of-distribution samples, we will then just use the positive model. This obviously leads to a question of how to determine whether a given sample is in or out of distribution \citep{9144212, choi2019waic}. During testing, our method ensembles the positive model, the negative model, and the discriminative model based on the degree of the similarity of the test sample to the training samples, and found that this works well for our purpose.} We measure this degree of similarity with probability cumulative density function (cdf) in terms of perplexity \citep{DBLP:journals/corr/abs-1812-04606}.

In the field of contrastive and self-supervised learning~\cite{DBLP:journals/corr/abs-2006-07733, DBLP:journals/corr/abs-2103-03230, DBLP:journals/corr/abs-2105-04906}, it is well known that just training on positive samples alone can lead to a degenerate solution, e.g., a constant function network would still produce a perfect training loss. To prevent this, we propose a novel generative framework where we use an autoregressive transformer, specifically BART \citep{DBLP:journals/corr/abs-1910-13461}. 
%While we have different choices such as contrastive learning~\cite{}, metric learning~\cite{}, we found that our proposal outperforms these methods. \snl{Yifei, can we run comparisons to constrative/metric learning?} %
Given two sentences, we condition the prediction of the next token in the second sentence on the first sentence and the previous tokens. In a Bayesian sense, this would mean that the next token predicted has a higher probability of being a positive/negative pair to the first sentence for the positive and negative model respectively. This learning strategy has no conceivable degenerate solutions even when we are training the positive and negative models separately.

In summary, our contributions are as follow:
\begin{enumerate}
    \item We report new research insights, supported by empirical results, that the negative pairs of a dataset could potentially introduce biases that will prevent a paraphrase identification model from generalizing to out-of-distribution samples.
    \item To overcome,  we propose a novel autoregressive modeling approach to train both a positive and a negative model, and ensemble them automatically during inference. We introduce a new perplexity based approach to determine whether a sample is out-of-distribution to achieve auto ensembling.
    \item We support our proposal with strong empirical results. Compared to state-of-the-art transformers in out-of-distribution performance, our model achieves an average of 11.5\% and 8.4\% improvement in terms of macro F1 and accuracy respectively over 7 different out-of-distribution scenarios. Our method is especially robust to paraphrase adversarials like PAWS, while keeping comparable performance for in-distribution prediction.
\end{enumerate}

==> introduction.tex <==

\section{Introduction}
Paraphrases are sentences or phrases that convey the same meaning using different wording \citep{10.1162/COLI_a_00166}. It is fundamental to the understanding of languages. Paraphrase Identification is the important task to identify if a pair of sentences has the same meaning, relevant to many applications such as summarization, machine translation, and question answering \citep{cer-etal-2017-semeval}.

Although recent works have shown great success in fitting to the distribution of individual datasets with various neural network architectures, achieving surprisingly high performances \citep{DBLP:journals/corr/WangHF17, DBLP:journals/corr/abs-1810-04805, DBLP:journals/corr/abs-2104-14690} on various datasets, those models can be especially fragile in face of distribution shift \citep{shen-lam-2021-towards}. A robust model for paraphrase identification is notoriously difficult. When the model trained from one source dataset $\mathcal{D}^t$is tested on another dataset $mathcal{D}^t$ collected and annotated independently, the classification accuracy drops significantly. In fact, as found by \citet{DBLP:journals/corr/abs-1904-01130}, by some adversarial examples, the accuracy can immediately drop to around the chance level (50\%). 

Previous works studying distribution shift in NLP blame the poor performance of generalizing to other datasets on the issue of shortcut learning \citep{DBLP:journals/corr/abs-1803-02324, DBLP:journals/corr/abs-2004-07780}, where unexpected clues introduced in the process of dataset collection and annotation is learned by the model to help make predictions. Making use of those shortcut features cannot generalize to real-world out-of-distribution scenarios. Previous works \citep{DBLP:journals/corr/abs-2103-06922, DBLP:journals/corr/abs-1908-10763, DBLP:journals/corr/abs-1909-03683} propose to identify training samples with more shortcut features and reduce the reliance of their models on short features to mitigate shortcut learning in Natural Language Inference tasks, but their methodology requires to hand-pick some shortcut features from known dataset bias \citep{DBLP:journals/corr/abs-1909-03683}, which is sometimes insufficient and even impractical. Especially in the case of paraphrase identification, it can be difficult to find exactly the specific dataset bias feature learnt by the black-box paraphrase identification models.

A key motivation for our methodology is the observation that those negative examples (i.e. non-paraphrase pairs) in common paraphrase identification datasets only represent a limited perspective of how the meanings of sentences can be different (and indeed it is pratically infeasible to represent every possible perspective). As illustrated in Figure~1, Quora Question Pair (QQP) \footnote{https://quoradata.quora.com/First-Quora-Dataset-Release-Question-Pairs} extracts its negative samples from similar topics. Paraphrase Adversarials from Word Scrambling (PAWS) \citet{DBLP:journals/corr/abs-1904-01130} generate negative examples primarily from word swapping. Microsoft Research Paraphrase Corpus (MSRP) extracts negative samples from news clusters. We therefore hypothesize that those biased hard negative mining strategies of common paraphrase identification datasets are major causes of the poor generalizability of various paraphrase identification models.

\begin{figure}[h!]
    \centering
    \includegraphics[width=.5\textwidth]{negative examples.pdf}
    \caption{An illustration of negative samples in different datasets.}
    \label{linreg}
\end{figure}

Intuitively, we would like to control the reliance on negative examples for out-of-distribution prediction. However, this is difficult with discriminative training.\snl{why is this difficult with discriminative learning but ``therefore'' easy with autoregression?} Therefore, we propose a novel generative framework where we use two  autoregressive transformers, specifically BART \citep{DBLP:journals/corr/abs-1910-13461}, to separately fit to different distributions of positive examples and negative examples. In this way, we can separate the reliance on positive examples and negative examples. While testing, those two models can be ensembled according to either Bayesian Inference Law or the degree of the similarity of the test example to the training example. \snl{bayesian blah blah or degree of blah blah make no sense, rewrite} We measure this degree of similarity with probability cumulative density function (cdf) in terms of perplexity.\snl{Is perplexity our work or existing work. if former, we need to motivate more, if latter, cite} 

On all 6 different combinations of QQP, PAWS, and MSRP, our generative model shows significant improvements in terms of out-of-distribution prediction with around 10\% gain in both ROC-AUC score and accuracy, while keeping the performance of our model for in-distribution prediction comparable to the state-of-the-art methods.

In brief, our contributions are twofold:
\begin{enumerate}
    \item We propose a novel generative framework for paraphrase identification to train two models to fit to the distribution of positive examples and negative examples separately. Models are assembled only while testing with controlled reliance on negative examples. Our model achieves an average of 9.4\% and 10.4\% improvement of ROC-AUC score and accuracy respectively over 6 different combinations of paraphrase datasets over state-of-the-art transformer methods in terms of out-of-distribution performance, especially robust to paraphrase adversarials like PAWS, while keeping comparable performance for in-distribution prediction.
    
    \item In addition to Bayesian Inference Law, we come up with a novel\snl{what do you mean in addition to bayesian inference law?} out-of-distribution based model to control reliance on negative samples. We design experiments to verify that the biased hard negative mining strategies of common paraphrase identification datasets are significant sources of poor generalizability for paraphrase identification. Controlled reliance of our model on negative samples increases the generalizing performance. 
\end{enumerate}

==> related_bak.tex <==
\section{Related Works} 
\subsection{Distribution Shift and Debiasing Models in NLP}
Previous works have also various proposed model ensembling methods to reduce the reliance on dataset bias \citep{DBLP:journals/corr/abs-1908-10763, pmlr-v119-bahng20a, DBLP:journals/corr/abs-1906-10169, DBLP:journals/corr/abs-1909-03683, DBLP:journals/corr/abs-2009-12303} for better performances in terms of distribution shift, mostly in the fields of Natural Language Inference, Visual Question Answering, and Question Answering. Their models share the same paradigm where they define the samples $x$ to contain signal features $x_s$ and biased features $x_b$, with the hope to prevent their model from relying on $x_b$ to make predictions that cannot generalize to out-of-distribution samples \cite{pmlr-v119-bahng20a}. To achieve this goal, they first attain a biased model which is hoped to make predictions only based on biased features $x_b$, either by known dataset bias \citep{DBLP:journals/corr/abs-1906-10169, DBLP:journals/corr/abs-1909-03683, DBLP:journals/corr/abs-1908-10763} or models with limited abilities not capable of capturing complicated semantic features desired as $x_s$. Then they train their main model for prediction with a regularization term to make their main model deviated from the results given by the biased model. Only the main model is used for testing.

However, this type of model ensembling methods show little success in debiasing paraphrase identification models, potentially because it is hard to point out the specific shortcut features in this task, as we shall see in Section 4. Our method differs from theirs in that we identify the source of dataset bias to be biased hard negative mining strategies instead of shortcut features. Our model ensembling methodology seeks to appropriately make use of the more biased model instead of deviating from it.

\subsection{Out-of-distribution Detection}
Another line of work relevant to this paper is the task of Out-of-distribution Detection, which aims to automatically distinguish samples that are out of some certain distribution we care about \citep{9144212}. Some of the methods seek to detect anomaly examples by examining the softmax scores \citep{DBLP:journals/corr/LiangLS17} or energy scores \citep{DBLP:journals/corr/abs-2010-03759} outputted by the discriminative model, others take a probabilistic approach to estimate the probability density \citep{choi2019waic, DBLP:journals/corr/abs-1812-04606}. In this paper, we consider a situation even more challenging than detecting out-of-distribution samples, where we seek to ensemble models in consideration of the degree of similarity of the sample with the training distribution. Our methodology differs from previous probabilistic approaches in that instead of just estimating the probability density, we estimate the cumulative density function as weights for model ensembling.
